OpenDeepThink: Parallel Reasoning via Bradley-Terry Aggregation

Test-time compute scaling is a primary axis for improving LLM reasoning. Existing methods primarily scale depth by extending a single reasoning trace. Scaling breadth by sampling multiple candidates in parallel is straightforward, but introduces a selection bottleneck: choosing the best candidate without a ground-truth verifier, since pointwise LLM judging is noisy and biased. To address this, we introduce OpenDeepThink, a population-based test-time compute framework that selects via pairwise Bradley-Terry comparison. Each generation, the LLM judges random pairs of candidates and aggregates votes via Bradley-Terry into a global ranking; top-ranked candidates are preserved and the top three quarters are mutated using the natural-language critiques produced during comparison; the bottom quarter is discarded. OpenDeepThink raises Gemini 3.1 Pro's effective Codeforces Elo by +405 points in eight sequential LLM-call rounds (~27 minutes wall-clock). The pipeline transfers across weaker and stronger models without retuning, and on the multi-domain HLE benchmark, gains appear concentrated in objectively verifiable domains and reverse in subjective ones. We release CF-73, a curated set of 73 expert-rated Codeforces problems with International Grandmaster annotation and 99% local-evaluation agreement against the official verdict.

==> packages.tex <==
%% packages.tex —— 全部 LaTeX 包的统一入口
%% 由 MITcsail.cls 在 \LoadClass 之后 \input 进来
%% 顺序：math → 排版/字体 → 颜色 → 图 → caption → 表格 → 布局 → 工具 → 算法 → bib → hyperref（最后）

%%==================== Math ====================
\RequirePackage{amsmath}
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{mathtools}
\RequirePackage{bm}
\RequirePackage{mathpazo}

%%==================== 排版 / 字体 ====================
\RequirePackage{microtype}
\RequirePackage{anyfontsize}
\RequirePackage{titlesec}

%%==================== 颜色 ====================
\RequirePackage[dvipsnames]{xcolor}
\RequirePackage{colortbl}

%%==================== 图与排版插入 ====================
\RequirePackage{graphicx}
\RequirePackage{svg}
\RequirePackage{wrapfig}
\RequirePackage{adjustbox}
\RequirePackage{tikz}

%%==================== Caption ====================
\RequirePackage[labelsep=colon]{caption}
\RequirePackage{subcaption}

%%==================== 表格 ====================
\RequirePackage{booktabs}
\RequirePackage{multirow}
\RequirePackage{tabularx}
\RequirePackage{tabu}
\RequirePackage{makecell}

%%==================== 布局 ====================
\RequirePackage{fancyhdr}
\RequirePackage{authblk}
\RequirePackage{enumitem}
\RequirePackage{tcolorbox}
\tcbuselibrary{breakable,skins}

%%==================== 工具 ====================
\RequirePackage{datetime}
\RequirePackage{verbatim}
\RequirePackage{lipsum}
\RequirePackage{pifont}

%%==================== 算法 ====================
%% opendeepthink 使用 algorithmicx 语法（\Require / \State / \For 等），加载 algorithm + algpseudocode
\RequirePackage{algorithm}
\RequirePackage{algpseudocode}
\RequirePackage{nicefrac}

%%==================== Bib ====================
\RequirePackage{natbib}

%%==================== Hyperref（必须最后加载）====================
\RequirePackage[colorlinks=true,citecolor=blue,linkcolor=black]{hyperref}
\RequirePackage[capitalize,noabbrev]{cleveref}

